Fooling End-to-end Speaker Verification by Adversarial Examples

Automatic speaker verification systems are increasingly used as the primary means to authenticate costumers. Recently, it has been proposed to train speaker verification systems using end-to-end deep neural models. In this paper, we show that such systems are vulnerable to adversarial example attack. Adversarial examples are generated by adding a peculiar noise to original speaker examples, in such a way that they are almost indistinguishable from the original examples by a human listener. Yet, the generated waveforms, which sound as speaker A can be used to fool such a system by claiming as if the waveforms were uttered by speaker B. We present white-box attacks on an end-to-end deep network that was either trained on YOHO or NTIMIT. We also present two black-box attacks: where the adversarial examples were generated with a system that was trained on YOHO, but the attack is on a system that was trained on NTIMIT; and when the adversarial examples were generated with a system that was trained on Mel-spectrum feature set, but the attack is on a system that was trained on MFCC. Results suggest that the accuracy of the attacked system was decreased and the false-positive rate was dramatically increased.

==> related_work.tex <==
\textbf{Speaker verification.} Past works focused on speaker verification presented methods of training several independent components (GMM,iVectors,SVM) to solve the problem, these components are not jointly optimized. Recently, more works approach the aforementioned problem with deep neural models \cite{snyder2016deep} \cite{zhang2016end} \cite{heigold2016end}, proposing an end-to-end optimization using a single unifying model. These models use neural networks as features extractors, providing with a representation on the utterance level. This representation is usually achieved by feeding a sequence with the help of some recurrent unit such as LSTM \cite{hochreiter1997long} or GRU \cite{DBLP:journals/corr/ChungGCB14}.
\\ \\
\textbf{Adversarial examples.} The empirical study of ~\cite{szegedy2013intriguing} first demonstrated that deep neural networks could achieve high accuracy on previously unseen examples while being vulnerable to small adversarial perturbations. This finding has recently aroused keen interest in the community~\cite{goodfellow2015explaining,papernot2016practical,szegedy2013intriguing,tabacof2015exploring}. Several studies have subsequently analyzed the phenomenon~\cite{fawzi2015analysis,shaham2015understanding,fawzi2016robustness} and various approaches have been proposed to improve the robustness of neural networks~\cite{papernot2016distillation,cisse2017parseval}. 
More closely related to our work are the different proposals aiming at generating better adversarial examples~\cite{goodfellow2015explaining,moosavi2015deepfool}. 
